Segmenting Low-Contrast XCTs of Concrete: An Unsupervised Approach

X-Ray Computed Tomography (XCT) is a compelling tool in experimental mechanics, capable of non-destructively extracting information pertaining to the internal morphology of materials. For materials with random heterogeneous morphology such as concrete, such information is of particular relevance since it allows for studies of morphology-related behaviour and for predictive modelling. Nevertheless, XCT images require semantic segmentation for practical usage. Here, concrete poses a unique challenge due to the similar X-ray attenuation coefficients of aggregates and mortar, which result in low contrast between the two phases in the ensuing XCT images. As such, purely intensity-dependent semantic segmentation tools remain unfeasible. While vision transformers (ViTs) and convolutional neural networks (CNNs) are proven techniques for semantic segmentation in such challenging cases, they typically require labelled training data, which is often unavailable for concrete or resource-intensive to obtain, thereby limiting their relevance. To address this challenge, a self-annotation technique is presented here that leverages superpixel algorithms to identify perceptually similar local regions in an image and relates them to the global context by utilizing the receptive field of a CNN-based model. This enables the model to learn a global-local relationship in the images and facilitates the identification of semantically similar structures. When evaluated against manually annotated ground truth on out-of-distribution data, the proposed methodology consistently outperformed direct greyscale thresholding across all pertinent metrics, demonstrating improved discernibility between aggregates and mortar, and providing the most favourable balance of sensitivity and precision for aggregate-phase identification.

==> math_commands.tex <==
% Sets
\RequirePackage{mathtools}
% \usepackage{mathalpha}
% \mathbcal{ABC}

\newcommand{\realNum}{\mathbb{R}}
\newcommand{\naturalNum}{\mathbb{N}}
\newcommand{\integer}{\mathbb{Z}}
\newcommand{\integerNN}{\mathbb{Z}_+}

\newcommand{\set}[1]{\boldsymbol{\mathcal{#1}}}

% Tensor 
\newcommand{\tensor}[1]{\boldsymbol{\mathrm{#1}}}
\newcommand{\tensorComp}[1]{\mathrm{#1}}
\newcommand{\scalar}[1]{\mathrm{#1}}


% Operators
\newcommand{\diff}[1]{\mathrm{d}{#1}}

% Functions
\newcommand{\scalFunc}[1]{{\mathscr{#1}}}
% \newcommand{\scalFunc}[1]{{\mathbcal{#1}}}
\newcommand{\tensorFunc}[1]{\boldsymbol{\mathscr{#1}}}
% \newcommand{\tensorFunc}[1]{\boldsymbol{\mathbcal{#1}}}

\DeclareMathOperator*{\argmax}{arg\,max}

